ShapeNet: An Information-Rich 3D Model Repository

We present ShapeNet: a richly-annotated, large-scale repository of shapes represented by 3D CAD models of objects. ShapeNet contains 3D models from a multitude of semantic categories and organizes them under the WordNet taxonomy. It is a collection of datasets providing many semantic annotations for each 3D model such as consistent rigid alignments, parts and bilateral symmetry planes, physical sizes, keywords, as well as other planned annotations. Annotations are made available through a public web-based interface to enable data visualization of object attributes, promote data-driven geometric analysis, and provide a large-scale quantitative benchmark for research in computer graphics and vision. At the time of this technical report, ShapeNet has indexed more than 3,000,000 models, 220,000 models out of which are classified into 3,135 categories (WordNet synsets). In this report we describe the ShapeNet effort as a whole, provide details for all currently available datasets, and summarize future plans.

==> notes.tex <==
%!TEX root = main.tex
\angel{Rewrite to indicate that current release only include designed models.  But that there will be more and more scanned models, so we also plan to incorporate those in our dataset in the future.}
Our initial intent is to collect 3D models from a wide variety of online repositories, described with a variety of shape representations (polygonal meshes, point clouds, CSG, voxels, etc.), and stored in a range of industry-standard file formats (COLLADA, Wavefront OBJ, PLY, etc.). 

We intend to support both ``designed'' 3D models as well as ``acquired'' ones, including multi-view RGBD data, which will be a more common 3D data source in upcoming years, as RGBD cameras become prevalent. Whenever possible, ShapeNet will provide basic tools for converting between these shape representations and file formats. Future research projects may also enhance this functionality.

\mypara{Internal structural properties:}
\begin{itemize}\denselist
  \item {\em Hierarchical part decompositions:} Each model is annotated not only with its top-level category labels, but also with a hierarchical decomposition of its surface into labeled parts.  For example, the surface of a swivel chair might be decomposed into subsurfaces representing the back, seat, arms, and leg. These subsurfaces may be divided further, e.g., the swivel leg is decomposed into leg base, leg column and leg mechanism. Each part is tagged with a reference to the WordNet synset representing the part, if one exists. These part decompositions serve as the building blocks for many applications such as shape modeling/synthesis, understanding shape structures, and computing abstractions for visualization. They also provide links between WordNet synsets. For example, a ShapeNet query to retrieve all wheels can return not only the models representing one wheel, but also all the parts of models that have been identified as wheels in the hierarchical decomposition.
  \item {\em Symmetries:} Many real-world objects exhibit symmetries, (e.g., planar reflectional symmetries, $k$-fold rotational symmetries, etc.), which are useful to maintain as the model is edited \cite{Golovinskiy:2009:symmetry-aware}, leverage when finding correspondences \cite{Liu:2012:finding}, and/or guide physical interactions with other objects.  Accordingly, ShapeNet will provide descriptions (e.g., a reflection plane) for a discrete set of prominent perfect, partial, and/or approximate symmetries for each model. In our current status, we will provide perfect symmetries.
\end{itemize}

\mypara{Physical properties:}
\begin{itemize}\denselist
  \item {\em Materials:} The material properties of 3D models are important for many applications, including rendering, recognition, and physical simulation. Accordingly, parts of models in ShapeNet will be annotated accordingly, with references to the physical materials used in their construction, whenever those can be determined.  For example, the entirety of an IKEA chair might be labeled with ``pine wood,'' or a fancy dining room chair might have labels of ``mahogany wood'' on the legs and back and ``foam, fabric'' on the seat. As a starting point, we will consider only surface materials. However, construction materials could be added as the repository evolves.
  \item {\em Weight, Strength, etc.:} Physical properties of 3D models are also very valuable for simulations and for reasoning about object uses, 3D printing and manufacturing, object participation in assemblies, etc.. For example, when composing a scene, it might be important to know how much an object weighs, how much weight in can bear, where its center of mass is, its brittleness, its deformation modes, etc. Such properties might be available from the model source or, in some cases, it might be possible to estimate thm from simulations, images or videos.
  \item {\em Appearance:} Whenever available, we also record, color, texture, and other appearance information.
\end{itemize}

\mypara{External interaction and placement properties:}
\begin{itemize}\denselist
  \item {\em Contact relationships:} Knowing how a model typically is in contact with other objects is useful for placing it into a scene and reasoning about how it is affected by changes to other models in a scene. Specifically, we augment each model by marking regions typically in contact with its supporting environment (e.g., tips of the legs of a desk) and regions suitable for supporting other objects (e.g., the flat surface on the top of a desk).
  \item {\em Affordances:} Knowing how people usually interact with a 3D model (i.e., which parts of a human body come in contact with which points on the 3D surface) is useful for predicting functions and ergonomics of an object~\cite{gibson:1977:theory}, reasoning about navigation through a scene~\cite{heft:1996:navigation,sun:2007:workspaceErgonomics}, and guiding algorithms that process the model to maintain properties important for human use~\cite{kuo:2005:ergonomicEvaluator, Jiang13}.  Accordingly, we augment each model with a discrete set of human poses and human-surface contact points representing likely interaction modalities.
  \item {\em Canonical views:} Knowing how people typically view a model is useful for generating representative images (e.g., thumbnails), reasoning about surface saliency (e.g., what people typically see), and guiding model processing (e.g., simplification) \cite{secord:2011:perceptual}.  Accordingly, we plan to provide a discrete set of ``canonical views'' for each model.
\end{itemize}


Rather than being a repository of individuals, as a prominent feature (and to justify the ``Net'' in its name), ShapeNet records relations and provides correspondences between 3D models and links to other sources of correlated data. These correspondences enable a wide range of applications, such as transferring annotations, analyzing and detecting shared structures, understanding property variations within a category, and designing exploration and visualization tools.

\mypara{Correspondence Annotations:}
\begin{itemize}\denselist
  \item {\em Model-model correspondences:}\hao{perhaps remove this part, or signficantly down-tune this part.} As a core feature, ShapeNet will include correspondences between surfaces of models within the same (or related) categories. These correspondences enable a wide range of applications, including propagating attributes across shapes, joint shape understanding~\cite{hwg-fmnaelsc-14} and shape exploration~\cite{kim:2012:fuzzycorres,hwg-fmnaelsc-14}. Based on the characteristics of shapes, we consider three types of correspondences that are meaningful in the context: dense point-wise correspondences, part-wise correspondences and sparse region-wise correspondences. Point-wise correspondences are suitable for shapes that are very similar to each other, e.g., between two human models. Part-wise correspondences exist among diverse shape collections that exhibit structural similarities, e.g., between two chair models. Region-wise correspondences are used to capture relations across categories, e.g., contain contact regions of human hands/legs on various models (bicycles, chairs, keyboards). These correspondences can be established using a variety of extant techniques, using geometric shape descriptors, whole shape alignments \cite{KaickZHC11} and joint correspondence optimization among a collection of shapes~\cite{kim:2012:fuzzycorres,hg-csmsdp-13,hwg-fmnaelsc-14}. To control the quality of the resulting correspondences, we incorporate user-specified correspondences as constraints when optimizing correspondences.
  
  %For models with hierarchical part decompositions, there will be annotations representing part-part correspondences.  Within each leaf part, ShapeNet will aim to establish point-to-point correspondences, whenever that is semantically meaningful. For example, given a distinctive point at the corner of a rectangular seat on one chair, it should be possible to find semantically corresponding point(s) on other chairs with rectangular seats \attn{(Figure XXXa)}.
  
  \item {\em Model-image correspondences:} It will be valuable to establish links from ShapeNet to data sources outside of ShapeNet that provide complimentary representations of the same objects or scenes. For example, linking images from ImageNet to objects in ShapeNet will be very valuable for learning about the appearances of 3D surfaces and shapes in images. To support these features, we will provide mechanisms to encode correspondences between pixels in images and points on 3D surfaces.
  
  A preliminary version of this effort was introduced in \cite{xiang:2014:pascal3d} where we presented a new dataset called PASCAL3D+. In this dataset, we augmented 12 rigid categories in the PASCAL VOC 2012 dataset \cite{everingham2010pascal} with 3D annotations. Specifically, for each object category we selected a number of CAD models from the Trimble 3D Warehouse. These CAD models were selected so as to include a large degree of intra-class variability for each category. Moreover, for each CAD model, an annotator identified a number of distinctive feature points or    landmarks    (e.g., for the car category, examples of landmarks
  are the center of a wheel, the top-left corner of a windshield, etc.). Then, the annotator followed two main steps: i) for each image and for each object in the image, the object was associated to the closest CAD model; ii) for each CAD model, the landmark points on the CAD model were associated to the corresponding 2D locations of the object in the image (if visible). By using these 3D-2D correspondences, we automatically aligned the CAD model to the object in the image and computed accurate 3D pose information.
  % This original dataset was further augmented by including images from the ImageNet dataset \cite{deng:2009:imagenet} for each of the 12 categories introduced above.
  An illustration of this annotation process and some examples of registrations between CAD models and images of objects are shown in Fig~\ref{fig:imageshape}.
  % We plan on extending this effort to all of the object categories in ShapeNet and generalize the annotation tool so as to easily establish correspondences between millions of CAD models in ShapeNet and corresponding objects in image repositories such as ImageNet.
\end{itemize}

We note that in general point-to-point correspondences between shapes, or between shapes and images, may be impossible to establish due to large shape variations. In such cases correspondences can be represented probabilistically, using either fuzzy maps as in \cite{kim:2012:fuzzycorres}, or soft maps as in \cite{snbbg-smbs-12}. Even in the absence of exact correspondences, transfer of attributes between 3D shapes or shapes and images is possible, using the mechanism of functional maps \cite{fmapssig2012}, which includes the previous two as special cases. The PIs have developed a rich set of techniques that can be exploited here.

%Beyond collecting on-line data, we also plan to expand Shapenet to include models reconstructed from RGB/RGBD images. The PIs have developed a rich set of structure-from-motion and scan-based geometry reconstruction algorithms~\cite{Huang:2007:surfrecons,Huang:2010:foorplan,Xiao:2012:museum,Xiao:2013:sun3d}. We plan to apply these techniques to reconstruct xx-models and scenes from images and RGBD scans crawled from the internet. This is in the same spirit as internet-image based building reconstruction~\cite{Snavely:2006:phototourism}, but focuses on objects and scenes.


==> quality.tex <==
%!TEX root = main.tex
\ms{This section will probably be reworked since current results do not support the image size as quality hypothesis.}

Unlike images that are photographic recording of real world scenarios, most 3D models are manually designed. In practice, the quality of the 3D model meshes differs significantly in geometric detail, material fidelity and texture realism.

We believe that it is necessary and important to measure the quality of models in each aspect and provide this measurement as another useful attribute. For example, in geometry processing, high geometric detail is important but texture quality is often irrelevant. In contrast, for many vision applications models high quality materials and textures are important whereas low geometric detail is acceptable.

We propose a method to coarsely measure model quality by examining an approximation of the information content of rendered images. More concretely, for each model that has been aligned to a canonical pose, we render it at a set of predefined views evenly sampled on the viewsphere. We then save those rendered images to PNG files and calculate their total file size. This total size is used as a quality or detail-level measurement.  Since we use aligned models and choose the same set of views, the renderings are comparable rough estimates of the geometric or texture ``detail'' of a 3D shape from each view. This is due to the PNG image format compressing the original image data losslessly with the DEFLATE algorithm~\cite{roelofs:1999:png}, meaning its size can be regarded as a rough measure of image space entropy (i.e., ``detail'' or ``information'').

Following this scheme, we generate a geometry-only model quality measurement by rendering the model with no materials or textures.  We also generate a texture-sensitive model quality measurement by rendering the model with textures. The difference of the two can be viewed as the texture quality of the model.  This is a fairly coarse and na\"ive measurement but is a sensible approximation of model quality as demonstrated by the estimated quality ranking of car models in Figure~\ref{fig:quality_estimation}.  An important deficiency of this approach is that it cannot be reliably used to compare model qualities across object categories.  Furthermore, its resolution is only sufficient to separate very low quality models from reasonable quality models so ranking within the reasonable models is somewhat inconsistent.

<<<<<<< HEAD
% \ms{Consider only keeping one of quality estimation figures depending on how the results look}

%\begin{figure}[t]
%	\includegraphics[width=\linewidth]{./fig/placeholder.pdf}
%	\caption{Quality Estimation}
%	\label{fig:quality_estimation}
%\end{figure}
=======
\begin{figure}[t]
	\includegraphics[width=\linewidth]{./fig/placeholder.pdf}
	\caption{Quality Estimation}
	\label{fig:quality_estimation}
\end{figure}
>>>>>>> 052df160660bb9b9397233af7c36104d66f79dbd


==> rgbd-alignment.tex <==
%!TEX root = main.tex

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{fig/rgbd-alignment}
  \caption{\small{We collect a set of alignments of 3D models to RGB-D frames.}}
  \label{fig:rgbd-alignment}
\end{figure*}

We provide model to RGB-D alignment for models in ShapeNetCore and RGB-D images in SUN RGB-D. As shown in Figure~\ref{fig:rgbd-alignment}, using the bounding-box annotations provided by the SUN RGB-D dataset, for each object in a RGB-D image, we generate a list of models ranked by quantitative similarity measurements. Among the top candidates, a human worker can then select the most suitable models for each object.
First, for each annotated object in a scene, we identify a subset of candidate 3D models in ShapeNetCore that are of the same category. For each of the models in the subset, we compute a score that quantifies the similarity between the object point cloud defined by the 3D bounding box and the model.

In order to compute such a score, we use the size, orientation, and position information of the 3D bounding box annotation from SUN RGB-D as well as the scale and orientation information associated with each model from ShapeNetCore to resize, rotate, and translate the model. Then, we render the model using the same camera parameters as used to take the original photo, thereby generating a point cloud from the 3D model.

We then use a mutual similarity heuristic to generate a score for each model. We compute the distance transform of the real point cloud and sum the distance values corresponding to points that belong to the graphic model point cloud. This value indicates how well the real point cloud is ``explained'' by the 3D model. We then do the opposite to compute a sum of distance values that indicates how well the 3D model is matched by the real point cloud. By combining the similarity in both directions, we arrive at a score that captures the mutual similarity between the point cloud of an object and a 3D model.

For each object in an RGB-D scene, we compute the mutual similarity score of each 3D model, and rank the models accordingly. The models at the top of the list are most similar to the real object and thus suitable for generating synthetic data. Finally, we can have human workers select the best model from the top of the list, identifying the best alignment to the RGB-D image.


==> role.tex <==
%!TEX root = main.tex
\newtext{
ShapeNet is an open web repository of 3D model data, semantic annotations, and connections between the 3D shapes and other modalities such as images and text.  We believe that ShapeNet will prove to be an immensely useful resource to several research communities in several ways:

\mypara{Data-driven research} By establishing ShapeNet as the first large-scale 3D shape dataset of its kind we can help to move geometric analysis and computer graphics research toward a data-driven direction following recent developments in vision and NLP. Additionally, we can help to enable larger-scale quantitative analysis of proposed systems that can clarify the benefits of particular methodologies against a broader and more representative variety of 3D model data.

\mypara{Training resource} By providing a large-scale, richly annotated dataset we can also promote a broad class of recently resurgent machine learning and neural network methods for applications dealing with geometric data. Much like research in computer vision and natural language understanding, computational geometry and graphics stand to benefit immensely from these data-driven learning approaches.

\mypara{Benchmark dataset} We hope that ShapeNet will grow to become a canonical benchmark dataset for several evaluation tasks and challenges.  In this way, we would like to engage the broader research community in helping us define and grow ShapeNet to be a pivotal dataset with long-lasting impact.
}
